LiteVLoc: Map-Lite Visual Localization for Image Goal Navigation

This paper presents LiteVLoc, a hierarchical visual localization framework that uses a lightweight topo-metric map to represent the environment. The method consists of three sequential modules that estimate camera poses in a coarse-to-fine manner. Unlike mainstream approaches relying on detailed 3D representations, LiteVLoc reduces storage overhead by leveraging learning-based feature matching and geometric solvers for metric pose estimation. A novel dataset for the map-free relocalization task is also introduced. Extensive experiments including localization and navigation in both simulated and real-world scenarios have validate the system's performance and demonstrated its precision and efficiency for large-scale deployment. Code and data will be made publicly available.

==> doc/algorithm_vloc.tex <==
\begin{algorithm}[t]
  \caption{Hierarchical Visual Localization}
  \label{alg:visual_loc}
  \LinesNumbered
  \KwIn{Topological-Metric Map $\mathcal{M}=\{\mathcal{N}, \mathcal{E}\}$ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \
    Visual observations at time $k$: $\mathcal{Z}_{k}$\ \ \ \ \ \ \ \ \ \
    Motion measurements at time $k$: $\mathcal{U}_{k}$\ \ \ \ \ \ \ \ \ \
    Initial guess of the pose: $\breve{\mathbf{x}}_{k},\hat{\mathbf{x}}_{k-1}$\\}
  \KwOut{Estimated pose $\hat{\mathbf{x}}_{k}$\\}
  // \textit{Searching the Reference Keyframe}\\
  Extract visual features: $\mathbf{f}_{k} = F(\mathcal{Z}_{k})$\\
  \If{$\breve{\mathbf{x}}_{k}$ is not initialized}
  {
  Find the most similar node: $N_{ref} = Q(\mathbf{f}_{k}, \mathcal{N})$ \\
  Set the initial guess of the pose: $\breve{\mathbf{x}}_{k}=\mathbf{x}_{N_{ref}}$
  }\Else
  {
  Find the cloest node: $N_{c}=Q(\breve{\mathbf{x}}_{k}, \mathcal{M})$ \\
  Obtain covisible nodes: $\mathcal{N}_{vis}=Q(N_{c},\mathcal{E}_{N_{c}})$\\
  Find the most similar node: $N_{ref}=Q(\mathbf{f}_{k}, \mathcal{N}_{vis})$
  }
  // \textit{Determining the Metric Position}\\
  $\mathcal{K}_{ref},\mathcal{K}_{k}=$ \textit{MatchKeypoint}$(\mathcal{Z}_{ref}, \mathcal{Z}_{k})$\\
  $\mathbf{x}_{rel}=$ \textit{EstimateRelativePose}$(\mathcal{K}_{ref}, \mathcal{K}_{k}, \mathcal{Z}_{k})$\\
  Absolute pose in the world: $\hat{\mathbf{x}}_{k}=\mathbf{x}_{ref}\bigodot \mathbf{x}_{rel}$\\
  // \textit{Loosely Coupled Multi-Sensor Fusion}\\
  Update the pose: $\hat{\mathbf{x}}_{k}=$\\
\end{algorithm}

==> doc/bio.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Biography  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Biography  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Biography  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-1cm}
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/Peng.jpg}}]
%     {Peng Yin} received his Bachelor's degree from Harbin Institute of Technology, Harbin, China, in 2013, and his Ph.D. degree from the University of Chinese Academy of Sciences, Beijing, in 2018.
%     % He is a Post-doctoral researcher with the Robotics Institute at Carnegie Mellon University, Pittsburgh, USA.
%     He is currently an Assistant Professor at City University of Hong Kong, China.
%     His research interests include LiDAR SLAM, Place Recognition, 3D Perception, and Reinforcement Learning. Dr. Yin has served as a Reviewer for several IEEE Conferences ICRA, IROS, ACC, RSS.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/jjh.png}}]
%     {Jianhao Jiao} (Member, IEEE) received the B.Eng. degree in instrument science from Zhejiang University, Hangzhou, China, in 2017, and the Ph.D. from the Department of Electronic and Computer Engineering, the Hong Kong University of Science and Technology, Hong Kong, China, in 2021.
%     He is currently a senior research fellow with the Department of Computer Science, University College London.
%     His research interests include SLAM, 3D Perception, and Navigation.
%     Dr. Jiao is an Associate Editor of IEEE IROS 2024.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/shiqi.png}}]
%     {Shiqi Zhao} received his Bachelor's degree from Dalian University of Technology, Dalian, China, in 2018, and his Master's degree from the University of California San Diego, U.S., in 2020.
%     Currently, he is a PhD student at the City University of Kong Hong.
%     His research interests include Place Recognition, 3D Perception, and Map Merging System.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/lingyun.jpeg}}]
%     {Lingyun Xu} received her Bachelor's degree from Huazhong University of Science and Technology, Wuhan, China, in 2011, and her Ph.D. degree from the University of Chinese Academy of Sciences, Beijing, in 2018.
%     She is research Post-doctoral with the Department of the Robotics Institute, Carnegie Mellon University, Pittsburgh, USA.
%     Her research interests include Visual Tracking, SLAM, Place Recognition, 3D Perception, and Autonomous Driving. Dr. Xu has served as a Reviewer for several IEEE Conferences ICRA, IROS, CVPR, and ICCV.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/huaping_liu.jpeg}}]
%     {Huaping Liu} received the PhD degree from Tsinghua University, in 2004, and now he is a professor with the Department of Computer Science and Technology, Tsinghua University, Beijing, China. His research interests include robot perception and learning. 
%     He was a recipient of the National Science Fund for Distinguished Young Scholars.
%     He served as the area chair of Robotics Science and Systems for several times and currently He is senior editor of International Journal of Robotics Research.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/ghuang.jpg}}]
%     {Guoquan (Paul) Huang} (Senior Member, IEEE) received the B.S. degree in automation (electrical engineering) from the University of Science and Technology Beijing, China, in 2002, and the M.Sc. and Ph.D. degrees in computer science from the University of Minnesota--Twin Cities, Minneapolis, MN, USA, in 2009 and 2012, respectively. He currently is an Associate Professor of Mechanical Engineering (ME), Computer and Information Sciences (CIS), and Electrical and Computer Engineering (ECE), at the University of Delaware (UD), where he is leading the Robot Perception and Navigation Group (RPNG).  
%     % From 2012 to 2014, he was a Postdoctoral Associate with the MIT Computer Science and Artificial Intelligence Laboratory (CSAIL), Cambridge, MA, USA. His research interests focus on state estimation and spatial AI for autonomous vehicles and mobile devices, including probabilistic sensing, localization, mapping, perception and navigation of autonomous robots.
%     % Dr. Huang has received some honors and awards over the years, including the 2015 UD Research Award (UDRF), 2015 NASA DE Space Research Seed Award, 2016 NSF CRII Award, 2018 SATEC Robotics Delegation (one of ten US experts invited by ASME), 2018 Google Daydream Faculty Research Award, 2019 Google AR/VR Faculty Research Award, and the Winner for the IROS 2019 FPV Drone Racing VIO Competition. He was the recipient of the ICRA 2022 Outstanding Navigation Paper Award, and the Finalists of the RSS 2009 Best Paper Award and ICRA 2021 Best Paper Award in Robot Vision.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/milford_small.jpeg}}]
%     {Michael J. Milford}  (Senior Member, IEEE) received
%     the Bachelor of Mechanical and Space Engineering
%     degree and the Ph.D. degree in electrical engineering
%     from The University of Queensland, Brisbane, QLD,
%     Australia.
%     He was a Research Fellow on the Thinking Systems
%     Project with Queensland Brain Institute, in 2010.
%     Since 2010, he has been a Lecturer at the Queensland University of Technology (QUT), Brisbane,
%     QLD, Australia, where he is currently an Associate
%     Professor and an Australian Research Council Future
%     Fellow and the Chief Investigator of the Australian Centre of Excellence for
%     Robotic Vision. 
%     % His research interests include navigation across the fields of
%     % robotics, neuroscience, and computer vision.
%     % Dr. Milford was a recipient of an inaugural Australian Research Council
%     % Discovery Early Career Research Award in 2012. He has been a Microsoft
%     % Research Faculty Fellow since 2013.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/howie.jpeg}}]
%     {Howie Choset} received the B.S. Eng. degree in computer science and the B.S. Econ. degree in entrepreneurial management from the University of Pennsylvania (Wharton), Philadelphia, PA, USA, both in 1990, the M.S. and Ph.D. degrees in mechanical engineering from California Institute of Technology (Caltech), Pasadena, CA, USA, in 1991 and 1996, respectively.
%     He is currently a Professor of Robotics with the Carnegie Mellon University, Pittsburgh, PA, USA. His research group reduces complicated high dimensional problems found in robotics to low-dimensional simpler ones for design, analysis, and planning.
%     % Prof. Choset was elected as one of the top 100 innovators in the world under 35, by the MIT Technology Review, in 2002. In 2014, Popular Science selected his medical robotics work as the Best of What’s New in Health Care. 
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/basti.png}}]
%     {Sebastian Scherer} received his B.S. in Computer Science, M.S. and Ph.D. in Robotics from CMU in 2004, 2007, and 2010.
%     Sebastian Scherer is an Associate Research Professor at the Robotics Institute at Carnegie Mellon University. His research focuses on enabling autonomy for unmanned rotorcraft to operate at low altitude in cluttered environments. He is a Siebel scholar and a recipient of multiple paper awards and nominations, including AIAA@Infotech 2010 and FSR 2013. His research has been covered by the national and internal press including IEEE Spectrum, the New Scientist, Wired, der Spiegel, and the WSJ.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/han.jpg}}] {Jianda Han} (Member, IEEE) received the Ph.D. degree in mechatronic engineering from the Harbin Institute of Technology, Harbin, China, in 1998. From 1998 to 2003, he was a Visiting Scientist with the City University of Hong Kong, Hong Kong, China; Michigan State University, East Lansing, MI, USA; and Cornell University, Ithaca, NY, USA.
%     He is currently a Professor with the College of Artificial Intelligence, Nankai University, Tianjin, China, and the Institute of Intelligence Technology and Robotic Systems, Shenzhen Research Institute of Nankai University, Shenzhen, China. 
%     % His research interests include nonlinear estimation and control, robotics, and mechatronics systems.
% \end{IEEEbiography}


% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/ivan.jpeg}}]
%     {Ivan Cisneros} received his B.S. in Electrical Engineering with a minor in Computer Science from Harvard University in 2016.
%     He worked full time at NASA-JPL on several flight projects for 3 years before starting his graduate studies at Carnegie Mellon University. He is currently working on a Master's degree in Robotics within the Robotics Institute at CMU.
%     His research interests include SLAM, visual localization, 3D Perception, and Deep Learning.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/Abu.jpg}}]
%     {Abulikemu Abuduweili} received his B.S. in Electrical Engineering from Peking University, China, in 2017, and his M.S. in Electrical Engineering from Peking University, China, in 2020.  
%     He is currently a PhD student at Electrical Engineering and Robotics at Carnegie Mellon University, USA.
%     His research interests include Deep Learning, Robotics, and Computer Vision.
% \end{IEEEbiography}






% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/Changliu.jpg}}]
%     {Changliu Liu} received the B.S. degree in mechanical engineering and the B.S. degree in economics from Tsinghua University, China, in 2012, the M.S. degree in mechanical engineering, and the M.A. degree in mathematics from University of California, Berkeley, U.S.A., in 2014 and 2016 respectively, and the Ph.D. degree in mechanical engineering from University of California, Berkeley, U.S.A., in 2017. She is an assistant professor at the Robotics Institute at Carnegie Mellon University. Her research interests lie in the design and verification of intelligent systems with applications to manufacturing and transportation. She received NSF Career Award, Amazon Research Award, and Ford URP Award.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/zhang_ji.jpg}}]
%     {Ji Zhang} received his Ph.D. in Robotics from Carnegie Mellon University in 2017.
%     Ji Zhang is a Systems Scientist at the Robotics Institute at Carnegie Mellon University, where he leads in the development of a series of autonomous navigation algorithms. His work was ranked \#1 on the odometry leaderboard of KITTI Vision Benchmark between 2014 and 2021. He founded Kaarta, Inc, a CMU spin-off commercializing 3D mapping \& modeling technologies, and stayed with the company for 4 years as chief scientist.
%     His research interests are in robotic navigation, spanning localization, mapping, planning, and exploration.
% \end{IEEEbiography}




==> doc/extension.tex <==
\section{Rethink This Work}

The whole visual localization method is divided into mapping and localization modules. 
The mapping takes a set of images with poses from various sources as input $\mathcal{D}=\{(\mathcal{Z}_{j}, \hat{\mathbf{x}}_{j})\}$ (call segment), where $i$ is the id of the data capturing sequence, and outputs a map $\mathcal{M}$.
The definition of the map is a two-level topo-metric graph. But to be general, the $\mathcal{M}$ can be also implicitly represented by a neural model.
We formulate the incremental mapping process as follows
\begin{equation}
    \mathcal{M}_{k}
    =
    f(\mathcal{M}_{k-1}, \mathcal{D}^{'}),\ \ \ 
    \mathcal{D}^{'}
    =
    g(\mathcal{M}_{k-1}, \mathcal{D}),
\end{equation}
where $k$ indicates the iteration number when $k^{th}$ segment is included,
$f(\cdot)$ is the incremental mapping function that extracts necessary information of $\mathcal{D}$ (\textit{necessary} means optimal memory allocation while maximumly preserving the up-to-date environmental information),
and $g(\cdot)$ is the function to localize $\mathcal{D}$ into $\mathcal{M}_{k-1}$ and exploit the pose of $\mathcal{D}$ to jointly optimize poses in the original map.
The above process can be also used to describe the process of map update:
\begin{equation}
    \mathcal{M}_{new}
    =
    f(\mathcal{M}_{old}, \mathcal{D}^{'}),\ \ \ 
    \mathcal{D}^{'}
    =
    g(\mathcal{M}_{old}, \mathcal{D}).
\end{equation}


The online localization process uses $\mathcal{M}$ as the environmental representation to localize a new observation:
\begin{equation}
    \mathbf{x}_{i}, \Sigma
    =
    h(\mathcal{M}, \mathcal{Z}_{i}), \ \ \
    \mathcal{Z}_{i} = \{\mathbf{I}_{i}, \mathbf{D}_{i}\},
\end{equation}
where $h(\cdot)$ is the function to localize $\mathcal{Z}_{i}$ into $\mathcal{M}$. Some may argue whether there exists difference between $g(\cdot)$ and $h(\cdot)$. 
We explain there exist $3$ differences:
\begin{enumerate}
    \item $h(\cdot)$ takes depth information as input, while $g(\cdot)$ can only use color images. This is because many mobile devices do not have or provide distance of far objects.
    \item $h(\cdot)$ provides localization results of one frame, while $g(\cdot)$ provides localization results of a segment (i.e., multiple frames). And the prior poses of $\mathcal{D}$ can be used to improve results of $g(\cdot)$.
    \item The output uncertainty of $h(\cdot)$ can be further used for actively find a better localization position.
\end{enumerate}

The current paper presents these limitations which will be further considered in the next version:
\begin{enumerate}
    \item In mapping, this paper assumes that segment also provides depth information and manually provided initial pose, making the implementation of $g(\cdot)$ easier. But most of mobile devices cannot provide good depth information.
    \item In mapping, the implementation of $f(\cdot)$ defines ``information'' metric as the occupancy. But in practice, the ``information'' should be the number of landmarks.
    % \item In mapping, map update is not available.
    \item In localization, $h(\cdot)$ implements a hierarchical ``global-local'' localization strategy, which is not an end-to-end design and involves handcraft strategy to search for the most similar reference frame (as described in \cite{chen2024map}, the regressor is applied to a pair formed by an unseen query and an image from the mapping set using handcrafted strategy). This is very tricky.   
    % \item In localization, $g(\cdot)$ and $h(\cdot)$ are designed separately. 
    \item In localization, the robot is assumed that it always has valid localization and stays in the mapping region. The robot cannot navigation, or its navigation capability is limited to the region where it stays.
    \item Domain gaps, which exist among devices, and between the reference and query image, are not addressed.
    \item In navigation, the robot only uses a single-frame depth point cloud for motion planning, which tends to get stuck into local minimum.
    % \item More complex testing scenarios should be explored.
\end{enumerate}


==> doc/image/figure_pipeline_sling.tex <==
\begin{figure}[t]
    \begin{center}
        \includegraphics[width=0.9\linewidth]{Imgs/pipeline_sling.png}
    \end{center}
    \caption{}
    \label{fig:pipeline_vn}
\end{figure}


==> doc/image/figure_pipeline_vn.tex <==
\begin{figure}[t]
    \begin{center}
        \includegraphics[width=0.9\linewidth]{Imgs/pipeline_visual_navigation.png}
    \end{center}
    \caption{}
    \label{fig:pipeline_vn}
\end{figure}


==> doc/image/figure_solution_appearance_change.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \centering
  \subfigure[]{
    \label{fig:solution_appearance_change_place_modeling}
    \centering
    \includegraphics[width=0.245\textwidth]{Imgs/sec4/solution_appearance_change_place_modeling-crop}
  }
  % \hspace{-0.15cm}
  \subfigure[]{
    \label{fig:solution_appearance_change_place_matching}
    \centering
    \includegraphics[width=0.21\textwidth]{Imgs/sec4/solution_appearance_change_place_matching-crop}
  }
  \caption{Two typical solutions to appearance change. 
  (1) The i3dLoc system \cite{yin2021i3dloc} transforms panoramic images from the RGB color domain to the depth image domain, facilitating data association with LiDAR measurements. This method falls under the category of place modeling, as it explicitly models the 3D appearance of environments.
  (2) SeqNet \cite{Garg2021SeqNet} is categorized as a sequence-based method, as it involves comparing sequences of query images with sequences from a database of images.}
  \label{fig:solution_appearance_change}
  \vspace{-0.4cm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> doc/image/figure_vloc_scenario.tex <==
\begin{figure}[t]
  \centering
  \subfigure[Simulated Office]
  {\label{fig:vloc_real_street}\centering\includegraphics[width=0.135\textwidth]{Imgs/experiment/exp_vloc_simu_office-crop}}\hspace{-0.1cm}
  \subfigure[Street]
  {\label{fig:vloc_real_street}\centering\includegraphics[width=0.172\textwidth]{Imgs/experiment/exp_vloc_street-crop}}\hspace{-0.1cm}
  \subfigure[Crowded]
  {\label{fig:vloc_real_crowded}\centering\includegraphics[width=0.172\textwidth]{Imgs/experiment/exp_vloc_crowded-crop}}
  \caption{\rt{Visual localization method testing in different unseen environments (2 for simulated and 2 for real-world environments), indoor and outdoor, with various obstacle setups and lighting conditions.}}
  \label{fig:vloc_scenario}
  % \vspace{-0.3cm}
\end{figure}

==> doc/image/figure_vloc_traj_simulated.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.9\linewidth]{Imgs/place_holder.jpg}
  \end{center}
  \caption{\rt{Visual localization trajectory on simulated environments}.}
  \label{fig:vloc_scenario}
\end{figure}


==> doc/intro_mapping.tex <==
\subsection{Challenges}
In this paper, we consider that \textbf{vision-only image-goal navigation problem} and exploit data from mobile devices to construct a global navigation map.
The image-goal navigation problem is that the agent uses the constructed topological map to navigate from current observation to target observation. 
This will involve several challenges:
\begin{enumerate}
    \item Global Map Construction: To support flexible map update and storage during long-term operation, the map should be sparse and lightweight, while preserving necessary navigation information. 
    The map representation is the first issue.
    Another issue is that directly taking supervision from human users may be suboptimal for robot navigation. The map should be further refined according to traversability and surrounding obstacles.
    \item Global Localization: Localizing in the global map suffers from appearance change (\textit{e.g.,} change in objects and illumination) and viewpoint difference (\textit{e.g.,} difference between the view of the robot and mobile devices).
    \item Relative Localization or Distance Computation: Compute distance between current observation and next node.
    \item Local Navigation: Without precise prior information given by the global map, the local navigation should be flexible to handle cases such as path planning and static or dynamic obstacles avoidance; obtain the relative pose between the source image and subgoal image.
\end{enumerate}

\subsection{Contributions}
In this paper, we address these challenging by proposing a scalable navigation framework for mobile robot navigation.
We utilize the metric-topological map to represent the global environments, which is taken as a proxy to connect data from mobile devices to navigation.
The system possesses several advantages: 
(1) global mapping: low-cost, easy-to-maintain, and scalable;
(2) local navigation: robust against environmental changes and does not rely on real-time precise odometry.
In overall, this paper presents these following contributions:
\begin{enumerate}
    \item We propose a module to convert output of mobile devices (image and VIO results) into a topological map. 
    Since there is a difference between the trajectories of human users and those needed for robotic navigation, we refine the human trajectories as priors to obtain topological points suitable for robotic navigation.
    \item We developed a visual place recognition (PR) module to address diverse PR problems during navigation.
    \item We incorporated an iPlanner \cite{} as the unspervised path planning method to enable flexible navigation. This method inputs a 3D waypoint and depth image and outputs a collision-free path without using odometry.
\end{enumerate}
The system has been validated in simulated and real-world environments, covering indoor and outdoor scenarios.



==> doc/problem_statement.tex <==
\section{Preliminary}
\label{sec:problem_statement}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem Formulation of Visual Localization}
\subsubsection{Formulation}

\rt{TODO:} formulate the visual localization problem, using the basic probabilistic problem formulation

\begin{equation}
  \mathcal{X}^{*}
  =
  \underset{\mathcal{X}}{\arg\min}\ P(\mathcal{X} | \mathcal{Z})
  =
  \underset{\mathcal{X}}{\arg\min}\ P(\mathcal{X} | \mathcal{O}, \mathcal{M})
\end{equation}


We are given a set of images, we aim to construct a graph $\mathcal{G}=\{\mathcal{E}, \mathcal{N}\}$. Each node $\mathbf{n}_{i}\in\mathcal{N}$ contains the coordinates and descriptors. We need to propose the visual navigation system that use $\mathcal{G}$ as the map for achieving complete localization and planning.

\rt{TODO:} Different formulation of the map: Different from Place Recognition, Map-based Visual Localization, and Mine.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Discussion}
We recognize that there are several works in visual localization, while we are focusing on the metric-based visual localization.
The main differences between these works stand on the map representation and specific requirements of localization accuracy.
The visual place recognition (VPR) algorithms, such as NetVLAD, considering to determine the place where the robot is currently located, where the localization accuracy is up to a topological level (e.g., the place is a room or a corridor), with the telerance of several meters \cite{xu2021probabilisticvp}.
And the other categories are related to the map-based localization (e.g., 3D point clodu map, mesh, NeRF, and Gassuain Splatting), such as Hloc \cite{}, which aims to localize the camera in the map with the accuracy of several centimeters, with the wide application in AR.

Our works stand at the middle of these two categories, which aims to localize the robot in the map with the accuracy of several decimeters, with the main focus on scalable and long-term navigation, while providing metric-level localization to guarantee the performance of the visual navigation system.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Map Representation}
This paper builds upon the common definition of topological-metric map representation \cite{}, by proposing a two-level map for visual localization and motion planning, with different definitions of nodes and edges.
At each level, we use the undirected graph to represent the map, which is a graph $\mathcal{G}=\{\mathcal{E}, \mathcal{N}\}$, where $\mathcal{E}$ is the set of edges and $\mathcal{N}$ is the set of nodes. Each node $\mathbf{n}_{i}\in\mathcal{N}$ contains the coordinates. The edge $\mathbf{e}_{ij}\in\mathcal{E}$ contains the relative pose between two nodes $\mathbf{n}_{i}$ and $\mathbf{n}_{j}$.
The first level of the graph is used for visual localization, which it is called ``covisibility graph'', where two nodes are connected with edges if they are visible to each other.
And each node also stores the extracted features (e.g., descriptors) for the place recognition and image matching.
The second level of the graph is used for motion planning, where two nodes are connected with edges if they are reachable to each other (navigability).
And each node only contains the coordinates (i.e., $\mathbf{p}=[x,y,z]^{\top}$).

\rt{TODO: provide a figure to explain the graph-based representation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Algorithms of Hierarchical System}

Based on above disucssion, we propose the hierarchical solutions to solve the visual localization problem,
The overall pseudo code is shown in Algorithm \ref{alg:visual_loc}.
Section \ref{sec:methodology} will provide details of each module.

\rt{TODO}:
Fig. \ref{fig:overview_visual_loc} provides the overview of this hierarchical visual localization system.

\input{doc/algorithm_vloc.tex}


==> doc/related_work_vnav.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Visual Navigation}
Classicial metric-based navigation frameworks \cite{cao2022autonomous,wellhausen2021rough,yang2021real,zhou2023racer,chaplot2020learning,simon2023mononav}, have demonstrated effective and reliable performance in autonomous navigation in unseen terrains.
Their success is based on a modular framework that includes perception, mapping, and path searching.
They require the need to maintain a precise metric map, which increased overall latency and lack of robustness against noise or errors in real-world missions.
Navigation on topological maps simplifies the planning space and not sensitive to sensor noise \cite{}, where the enviornment is represented as a graph.
Topo-metric maps, which utilize the topological structure, while containing metric information, such as spatial coordinates \cite{}.
Several works \cite{} such as Kimera-Graph, first construct the compleet metric map, and then extract the topological structure based on free space from the map.
The resulting map, encoding visual features and semantics, showing desirable properties, has been integrated into reinforcement learning (RL) \cite{ravichandran2022hierarchical} or large language models (LLMs) to perform navigation tasks \cite{rana2023sayplan}.

There are other works directly construct the topological map on-the-fly \cite{chaplot2020neural}.
% teach-and-repeat
Several methods \cite{shah2023vint,he2023metric,sun2024fgprompt,sridhar2024nomad,suomela2024placenav} releases the reliance of metric localization, such as ViNT \cite{shah2023vint} and DeepExplorer \cite{he2023metric}.
They train an end-to-end navigation policy via. imitation learning (IL) or RL, which directly map sensory inputs to planning paths or control actions, given the current observation and the goal image.
But metric-free approaches almost entirely bypass the underlying geometric structure of the problem, while this information is available in practical robots such as the depth camera.
And as mentioned in \cite{yang2023iplanner,wasserman2023last}, both IL and RL methods are data hungry; IL method relies on having diverse data to function well in various scenarios, while RL truggles with low sampling efficiency and slow convergence.
The iPlanner \cite{yang2023iplanner} was proposed to explore a novel non-supervised imperative learning approach to train a planning policy from depth measurements end-to-end, sing differentiable metric-based optimization to direct
network updates.
It shows the usage of metric data, which is structured, to improve the learning efficiency.

This paper identifies the importance of metric information for reliable navigation and utilizes the topo-metric map for visual navigation.
The spatial coordinates, stored in the map, is used to guide the robot to the goal, enabling the usage of iPlanner, to further demonstrate the usage of our proposed VLoc for navigation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{enumerate}
  \item Image Retrieval: However, all these networks must discretise the world into places and are unable to produce a fine grained estimate of 6-DOF pose.
  \item Structure-based, using 3D map
  \item Structure-based with image retrieval, using 3D map
  \item Scene point regression, using 3D map or not: but scene-specific, each network needs to be trained given images and GT poses in this region: DSAC, ACE, ACEZero
  \item Absolute pose estimation, no using 3D map: PoseNet learns a mapping from pixel to high-dimensonal space linear with poses, trained with pose loss.
  \item Relative pose estimation, no using 3D map
  \item Pose interpolation, no using 3D map
\end{enumerate}
\end{comment}


\begin{comment}
\subsection{Metric Map-Centric Navigation}

\subsubsection{Geometric Methods}

Classic planning frameworks, such as those done by Cao et al. \cite{cao2022autonomous}, Wellhausen and Hutter \cite{wellhausen2021rough}, Yang et al. \cite{yang2021real}, have demonstrated effective and reliable performance in autonomous navigation in unseen terrains. For example, the navigation system, done by Cao et al. \cite{cao2022autonomous}, incorporating mapping, terrain analysis, and motion-primitive path search, is deployed successfully during the DARPA Subterranean Challenge.
The work of Wellhausen and Hutter \cite{wellhausen2021rough} employs a pipeline with a learned terrain estimator and executes a lazy-PRM path search, similar to the approach of Yang et al. \cite{yang2021real} who uses a learned terrain cost and performs PRM* with additional path optimization.
The modular framework, now, has been successfully applied the SOTA wheeled-legged robot
\footnote{\url{https://junja94.github.io/learning_robust_autonomous_navigation_and_locomotion_for_wheeled_legged_robots}}.

\subsubsection{Hybrid Geometric and Learning-Based Methods}
Recent advances in deep learning especially for the Large Language Models (LLMs) have enabled robots to perform more complex tasks which are not limited to waypoint navigation, including image-goal navigation, object-goal navigation, navigation to the goal which is described by language \cite{chang2023goat}, not event perform manipulation-navigation according to a language instruction as shown in SayPlan \cite{rana2023sayplan}.

The usage of \textbf{LLM} is progressive, and the LLM is beneficial to perception and planning.
Clip on Wheels (CoW) \cite{gadre2023cows} is proposed in which combines text and image caption models  with frontier-based exploration algorithms to perform object exploration in simulation.
The landmark-based navigation \cite{shah2023lm} is performed using pre-trained visual, language, and navigation modules.
LLM-Planner \cite{song2023llm} used the LLM to produce action sequences.
SayPlan \cite{rana2023sayplan} uses the LLM to generate high-level task plan with a pre-built 3D scene graph.
Voronav \cite{wu2024voronav} generates prompt by integrating both path descriptions and farsight descrptions, and utilizes LLM to predict semantic rewards for exploration in a object-goal navigation task.
NavCON \cite{biggie2023tell} focused on generating code using the code generation model \cite{chen2021evaluating} from language instructions that are compatiable to the downstream planning.
Shah \textit{et al.} \cite{shah2023navigation} takes the LLM as the search heuristic for planning during the exploration, by taking the advantage of LLM in infering objects' relationship, such as ``a kitchen often adjoins a living room, an exit sign indicates the way out''.
CLIO \cite{maggio2024clio} proposed the task-driven scene graph reconstruction, with the focus on specific objects.

The active neural SLAM \cite{chaplot2020learning} proposed the end-to-end reinforcement learning (RL) for exploration, under the assistance of a metric map.


% \subsubsection{End-to-End Planning}
iPlanner \cite{}: end-to-end planning, with the subsequent path following module to generate action.

\cite{ravichandran2022hierarchical} proposed the grapn neural network on the 3D scene graph.

RL \cite{hoeller2021learning}

Supervised Learning \cite{loquercio2021learning}

MonoNav \cite{simon2023mononav} proposed the monocular navigation framework by combining with ZoeDepth \cite{bhat2023zoedepth} for monocular depth estimation and traditionaly geometric planner.

\rt{While our work builds upon the existing literature on topological maps, the resemblance is only at high-level graph structure.
  Our work focuses on making visual topological mapping
  and exploration scalable, robust and efficient. We achieve
  this via the representation of both semantic and geometric
  properties in our topological maps; the ability to build topo-logical maps in an online manner and finally, posing the
  learning problem as a supervised problem.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Topological Map-Centric Navigation}

The topological map representation, recently, has been applied in image-goal navigation or field environment navigation.
The advantages of topological map are discussed in \cite{chaplot2020neural}.

\subsubsection{Methods Without Metric}
% Metric-Free
There are not distinct differences between the teach and repeat navigation task and image/object-goal navigation task.
The former commonly is applied to field robot navigation, where issues during the large-scale and long-term operation are considered.
The latter commonly considers the problem in indoor scenarios, with the goal to find the specific room/place or object.

\textbf{RL-based Methods}:
FGPrompt \cite{sun2024fgprompt} introduces a fine-grained prompting mechanism that preserves detailed information from the goal image and guides the observation encoder to focus on \textit{goal-relevant regions}, focusing on subgoal navigation.
The method employs a mid-fusion mechanism using FiLM \cite{perez2018film} layers for robust information exchange and an early fusion mechanism through joint modeling for implicit information exchange. With these input embeddings, FGPrompt trains a RL-based navigation policy.


\textbf{Imitation Learning:}
DeepExplorer \cite{he2023metric}

\textbf{Supervised Learning:}
GNM \cite{}

ViNT \cite{}

NoMaD \cite{sridhar2023nomad} proposed to use diffusion model to output distributions of action, trained with supervised data.

TSGM \cite{kim2023topological}

\subsubsection{Methods Using Metric}
But the above approaches almost entirely bypass the underlying geometric structure of the problem, while this information is available in practical robots such as the depth camera.
One can argue that the navigation can indeed be learned from data itself.
We agree that, in principle, it can be.
As emphasized in \cite{wasserman2023last}, however, we argue and demonstrate that an unstructured local policy for last-mile navigation is either
(1) sample inefficient (billions of frames in an RL framework) or
(2) biased and generalize poorly when learned from offline demonstrations (due to distributional shift).

SLING \cite{wasserman2023last} proposed the  image-goal navigation \textbf{benchmark} and demonstrated that the inclusion of geometric information significantly improves the performance.

The neural topological SLAM \cite{chaplot2020neural} proposed the topological representation, which is more scalable and robust to sensor noise.
Several key components are presented:
\textbf{Graph Update},
\textbf{Global Policy}, and
\textbf{Local Policy}.
Authors proposed the geometric explorable area prediction and semantic score prediction functions to predict high-level moving direction, and they further used the local policy module to output action.

\textbf{Self-Supervised Learning:}
In NRNS, a self-supervised approachach to learn to navigate from only passive videos of roaming was proposed as an exploratory navigation, by learning a generalizable distance estimator \cite{hahn2021no} in global policy. It use the local policy proposed in \cite{chaplot2020learning} to generate action.


\subsection{Visual Localization}

Topological Localization: \cite{xu2021probabilisticvp}, \cite{Xu2021ProbabilisticAT}

Metric Localization:

% \textbf{Teach and Repeat Navigation Task}: 
% Manually given topological node as the start and end.
% Recent works are are done withint the modular framework.

% \textbf{Image/Object-Goal Navigation Task}: 
% Manually given object and image, the agent should find the node.
% Recent works are done within the end-to-end framework. 
% In this framework, obstacles are not explicitly handled, directly generate action

% \subsection{Place Recognition Applications}

\subsection{Connection between Mobile Devices and Robots}
Mobile devices as sensors

SLAM/VIO

visual localization and mapping

\end{comment}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% - 基于几何地图的模块化导航
% - 基于几何地图的端到端导航
% - 基于拓扑地图的模块化导航（metric-topological map, topological map）
% - 基于拓扑地图的端到端导航（metric-topological map, topological map）
% - 基于几何地图-拓扑地图混合的导航
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> doc/table/table_dataset.tex <==
\begin{table*} [htbp]
  \centering
  \caption{Typical datasets for evaluating VPR, LPR, and RPR.}
  % Symbols \textbf{L}, \textbf{R}, \textbf{PinC}, and \textbf{PanC} indicate LiDAR, Radar, pinhole camera, and panoramas Camera respectively.
  % }
  \renewcommand\arraystretch{1.2}
  \renewcommand\tabcolsep{5pt}
  \begin{tabular}{r|c|c|c|c|c|c}
    \Xhline{0.03cm}
    \textbf{Dataset}
                                                 & \textbf{Scenarios}
                                                 & \makecell[c]{\textbf{Geographical}                                                                                                     \\ \textbf{Coverage}}
                                                 & \makecell[c]{\textbf{Sensors}}
                                                 & \makecell[c]{\textbf{Appearance}                                                                                                       \\ \textbf{Diversity}}
                                                 & \makecell[c]{\textbf{Viewpoint}                                                                                                        \\ \textbf{Diversity}}
                                                 & \makecell[c]{\textbf{Dynamic}                                                                                                          \\ \textbf{Diversity}}
    \\
    \Xhline{0.03cm}
    Nordland~\cite{sunderhauf2013we}             & Train ride                         & $748km$  & \text{PinC}                        & Four seasons                & \NoMark  & \NoMark  \\
    \Xhline{0.01cm}
    KITTI~\cite{DATASET:KITTI}                   & Urban Street                       & $1.7km$  & \text{L}, \text{PinC}              & Day-time                    & \NoMark  & \YesMark \\
    % \Xhline{0.01cm}
    % NCLT~\cite{DATASET:NCTL}                     & Campus                             & $5.5km$      & \text{L}, \text{PanC}              & Season                      & \YesMark & \NoMark  \\
    \Xhline{0.01cm}
    Oxford RobotCar~\cite{DATASET:Oxford}        & Urban + Suburban                   & $10km$   & \text{L}, \text{PinC}              & All kinds                   & \NoMark  & \YesMark \\
    \Xhline{0.01cm}
    Mapillary~\cite{warburg2020mapillary}        & Urban + Suburban                   & $4228km$ & \text{PinC}                        & All kinds                   & \YesMark & \YesMark \\
    \Xhline{0.01cm}
    KITTI360~\cite{DATASET:KITTI360}             & Urban Street                       & $73.7km$ & \text{L}, \text{PinC}, \text{PanC} & Day-time                    & \NoMark  & \YesMark \\
    \Xhline{0.01cm}
    % IndoorVPR~\cite{Liu2022indoordataset}        & Indoor                             & $0.0158km^2$ & \text{L}, \text{PinC},\text{PanC}  & Day-time                    & \YesMark & \NoMark  \\
    % \Xhline{0.01cm}
    ALTO~\cite{ivan2022alto}(States)             & Urban+Rural+Nature                 & $50km$   & Top-down \text{PinC}               & Day-time                    & \YesMark & \NoMark  \\
    \Xhline{0.01cm}
    ALITA~\cite{yin2022alita}(City)              & Urban + Terrain                    & $120km$  & \text{L}                           & Day time                    & \YesMark & \YesMark \\
    \Xhline{0.01cm}
    ALITA~\cite{yin2022alita}(Campus)            & Campus                             & $60km$   & \text{L}, \text{PanC}              & Day/Night                   & \YesMark & \YesMark \\
    \Xhline{0.01cm}
    Oxford Radar RoboCar \cite{barnes2020oxford} & Urban                              & $280km$  & \text{L}, \text{R}, \text{PinC}    & Day/Night, Weather, Traffic & \YesMark & \NoMark  \\
    % \Xhline{0.01cm}
    % \bt{MulRan} \cite{kim2020mulran}             & Urban                              & $xxx$       & \text{L}, \text{R}, \text{PinC}    & All kinds                   & \YesMark & \NoMark  \\
    % \Xhline{0.01cm}
    % GrAco \cite{zhu2023graco}                    & Campus                             & $7km$    & \text{L}, \text{PinC}              & Day-Time                    & \YesMark & \NoMark  \\
    % \Xhline{0.01cm}
    % WildPlace \cite{knights2023wild}             & Forest                             & $33km$       & \text{L}, \text{PinC}              & Day-Time                    & \YesMark & \NoMark  \\
    \Xhline{0.03cm}
    \multicolumn{7}{l}{\# \textbf{L}: LiDAR. \textbf{R}: Radar. \textbf{PinC}: Pinhole Camera. \textbf{PanC}: Panoramas Camera.}
  \end{tabular}
  \label{tab:public_datasets}
  \vspace{-0.3cm}
\end{table*}

==> doc/table/table_sensor_summary.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Contain related work (original version)
\begin{comment}
\begin{table*} [t]
  \centering
  \caption{Different Types of Camera Modalities}
  \renewcommand\arraystretch{1.2}
  \begin{tabular}{|C{3.5cm}|C{2cm}|C{11cm}|}
    \hline
    \textbf{Sensor}
                                       & \textbf{Related Work}
                                       & \textbf{Place Recognition Properties}
    \\
    \hline
    \textit{Partial-observable} Camera & \cite{Zaffar2020CoHoG,oertel2020augmenting,Khaliq2020RegionVLAD,ye2021visual,ozdemir2022echovpr,molloy2020intelligent,peng2021semantic,lu2021sta,waheed2021improving,khaliq2022multires,yuan2021softmp,piasco2021improving,mo2020fast,lee2021eventvlad}                                                   & These cameras are widely applied in most kinds of visual place recognition methods, but are sensitive to viewpoint differences, appearance changes, and dynamic objects.                  \\
    \hline
    \textit{Fully-observable} Camera   & \cite{yin2021i3dloc,yoon2014robust,lee2017fast,zioulis2021single,zhang2021panoramic,stone2016skyline,grelsson2020gps,liu2019lending}                                                                                                                                                                      & 360-degree cameras provide rich geometries, and can provide viewpoint (orientation)-invariant place recognition, but are sensitive to appearance changes and dynamic objects.             \\
    \hline
    LiDAR Device                       & \cite{Kim2018scancontext,guo2019local,zhu2020gosmatch,siva2020voxel,kim2020mulran,rozenberszki2020lol,komorowski2021minkloc3d,zywanowski2021minkloc3d,kim2021scan,yin2021pse,Yin2021spherevlad,vidanapathirana2021locus,yin2021fusionvlad,Xie2021RDC,li2022rinet,vid2022logg3d,lin2019fast,Wang2021Livox} & LiDAR provides the most accurate 3D environment measurements, and is invariant to appearance changes, but it usually has lower resolution and textureless inputs for confined/flat areas. \\
    \hline
    RADAR Device                       & \cite{gadd2020look,tang2020self,suaftescu2020kidnapped,gadd2021contrastive,cai2021autoplace,burnett2022radar,yin2021rall,hong2022radarslam}                                                                                                                                                               & Radar has 360-degree-view and not sensitive to both appearance and extreme weather conditions, but it has very low resolution inputs and noise cluster observations.                      \\
    \hline
    Joint Sensors                      & \cite{di2021visual,shan2021robust,yu2022mmdf,bernreiter2021spherical,cattaneo2020global,yin2021i3dloc,lai2021adafusion}                                                                                                                                                                                   & Joint sensors can cover the shortages of individual sensors, and the shared geometric property also make cross-modal place recognition methods possible.                                  \\
    \hline
  \end{tabular}
  \label{tab:sensor_summary}
\end{table*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Not contain related work
\begin{table*}[t]
  \centering
  \caption{Different Types of Camera Modalities}
  \renewcommand\arraystretch{1.2}
  % \scriptsize
    \begin{tabular}{|C{3.5cm}|C{2cm}|C{11cm}|}
      \hline
      \textbf{Sensor}
                                         & \textbf{Related Work}
                                         & \textbf{Place Recognition Properties}
      \\
      \hline
      \textit{Partial-observable} Camera & \cite{Zaffar2020CoHoG,oertel2020augmenting,Khaliq2020RegionVLAD,ye2021visual,ozdemir2022echovpr,molloy2020intelligent,peng2021semantic,lu2021sta,waheed2021improving,khaliq2022multires,yuan2021softmp,piasco2021improving,mo2020fast,lee2021eventvlad}                                                   & These cameras are widely applied in most kinds of visual place recognition methods, but are sensitive to viewpoint differences, appearance changes, and dynamic objects.                  \\
      \hline
      \textit{Fully-observable} Camera   & \cite{yin2021i3dloc,yoon2014robust,lee2017fast,zioulis2021single,zhang2021panoramic,stone2016skyline,grelsson2020gps,liu2019lending}                                                                                                                                                                      & 360-degree cameras provide rich geometries, and can provide viewpoint (orientation)-invariant place recognition, but are sensitive to appearance changes and dynamic objects.             \\
      \hline
      LiDAR                              & \cite{Kim2018scancontext,guo2019local,zhu2020gosmatch,siva2020voxel,kim2020mulran,rozenberszki2020lol,komorowski2021minkloc3d,zywanowski2021minkloc3d,kim2021scan,yin2021pse,Yin2021spherevlad,vidanapathirana2021locus,yin2021fusionvlad,Xie2021RDC,li2022rinet,vid2022logg3d,lin2019fast,Wang2021Livox} & LiDAR provides the most accurate 3D environment measurements, and is invariant to appearance changes, but it usually has lower resolution and textureless inputs for confined/flat areas. \\
      \hline
      RADAR                              & \cite{gadd2020look,tang2020self,suaftescu2020kidnapped,gadd2021contrastive,cai2021autoplace,burnett2022radar,yin2021rall,hong2022radarslam}                                                                                                                                                               & Radar has 360-degree-view and not sensitive to both appearance and extreme weather conditions, but it has very low resolution inputs and noise cluster observations.                      \\
      \hline
      % Joint Sensors                      & \cite{di2021visual,shan2021robust,yu2022mmdf,bernreiter2021spherical,cattaneo2020global,yin2021i3dloc,lai2021adafusion}                                                                                                                                                                                   & Joint sensors can cover the shortages of individual sensors, and the shared geometric property also make cross-modal place recognition methods possible.                                  \\
      % \hline
    \end{tabular}
  
  \label{tab:sensor_summary}
\end{table*}


==> doc/table/table_solution_to_challenge.tex <==
\begin{table*}[t]
  \centering
  \caption{Representative solutions to specific PR challenges.}
  \renewcommand\arraystretch{1.2}
  % \tiny
  % \footnotesize
  \begin{tabular}[t]{p{1.8cm}|p{15cm}}
    \Xhline{0.03cm}
    \textbf{Challenges}             &
    \textbf{Categories of Solutions}                                                                                                                       \\
    \Xhline{0.03cm}

    Appearance \newline Change      &
    \textbf{Place Modeling}: semantics \cite{peng2021semantic}, domain transfer \cite{yin2023isimloc}, event cameras \cite{lee2021eventvlad} \newline
    \textbf{Place Matching with Sequences}: sequence matching \cite{Milford2012SeqSLAM}, bayesian selection \cite{molloy2020intelligent}, dymaic time warping \cite{lu2021sta}
    \\
    \Xhline{0.01cm}

    Viewpoint \newline Difference   &
    \textbf{Geometric}: cylinder projection \cite{chen2021overlapnet,xu2021disco}, multi-view projection \cite{yin2021fusionvlad}, rotation-invariant descriptor \cite{komorowski2021minkloc3d} \newline
    \textbf{Appearance}: semantics \cite{garg2018don}, global descriptor \cite{relja2016netvlad,wang2022transvpr,ali2023mixvpr}, multi-scale feature fusion \cite{hausler2021patch} \newline
    \textbf{Others}: hybrid method \cite{yin2023automerge}, omnidirectional sensors \cite{yin2021i3dloc}
    \\
    \Xhline{0.01cm}

    Generalization \newline Ability &
    \textbf{Network Capability}: transformer \cite{wang2022transvpr}, foundation model \cite{keetha2023anyloc,oquab2023dinov2} \newline
    \textbf{Loss Functions}: rotation triplet \cite{Yin2021spherevlad}, angular \cite{loss:barros2021attdlnet}, divergence \cite{yin2021pse}, soft binary-cross entrpy \cite{li2022rinet} \newline
    \textbf{Incremental Learning}: loss functions \cite{gao2022airloop,knights2022incloud}, HMM \cite{doan2020hm}, dual-memory mechanism \cite{yin2023bioslam} \newline
    \textbf{Other Methods}: multi-modal information \cite{lai2021adafusion, komorowski2021minkloc++, paolicelli2022learning}, domain transfer \cite{yin2023isimloc}
    \\
    \Xhline{0.01cm}

    Efficiency                      &
    \textbf{Optimal Architecture}: efficient backbone \cite{sandler2018mobilenetv2,fan2022svt} \newline
    \textbf{Novel Network Design}: spiking neural network \cite{hines2023vprtempo} \newline
    \textbf{Non-Learning Method}: context encoding \cite{Kim2018scancontext}, planar features \cite{he2016m2dp} \newline
    \textbf{Effient Sequence Matching}: particle filter \cite{Fast_Yang}, approximate world's nearest neighbor \cite{Fast_Siam}, and HMM \cite{Fast_Peter} \\
    \Xhline{0.01cm}

    Uncertainty \newline Estimation &
    \textbf{Employed in PR}: MC Dropout \cite{gal2016dropout}, deep ensembles \cite{lakshminarayanan2017simple},
    probabilistic place embedding \cite{shi2019probabilistic}, self-teaching uncertainty \cite{cai2022stun} \newline
    \textbf{Employed in Other Tasks}: Laplace approximation \cite{yun2023laplace}
    \\

    \Xhline{0.03cm}
  \end{tabular}
  \label{tab:summary_solution_to_challenge}
  \vspace{-0.3cm}
\end{table*}


==> doc/table/table_survey.tex <==


\begin{table*} [t]
    \caption{Surveying the surveys and tutorials on place recognition}
    \centering
    \renewcommand\arraystretch{1.10}
    \renewcommand\tabcolsep{5pt}
    \begin{tabular}{|c|c|c|}
        \hline
        \textbf{Year}
         & \textbf{Topic}
         & \textbf{Reference}
        \\
        \hline
        \hline
        2015
         & Metric and Semantic SLAM
         & Cadena \textit{et al.} \cite{cadena2016past}
        \\
        \hline
        2015
         & Visual place recognition (position-based),
        three key modules: \textit{image processing, map, belief generation}, handcrafted features
         & Lowry \textit{et al.} \cite{lowry2015visual}
        \\
        \hline
        2021
         & Visual place recognition, deep learning approaches
         & Zhang \textit{et al.} \cite{zhang2021visual}
        \\
        \hline
        2021
         & Sensors and deep learning approaches: supervised, unsupervised, semi-supervised, parallel and hierarchical frameworks
         & Barros \textit{et al.} \cite{barros2021place}
        \\
        \hline
        2021
         & Visual place recognition (overlap-based),
        similar to content-based retrieval
         & Garg \textit{et al.} \cite{garg2021your}
        \\
        \hline
        2021
         & Visual place recognition, deep learning approaches
         & Masone \textit{et al.} \cite{masone2021survey}
        \\
        \hline
        2021
         & Visual place recognition benchmark: datasets, VRP methods, metrics, and evaluation
         & Zaffar \textit{et al.} \cite{zaffar2021vpr}
        \\
        \hline
        2023
         & LiDAR-based global localization
         & Yin \textit{et al.} \cite{yin2023survey}
        \\
        \hline
        2023
         & Active SLAM
         & Placed \textit{et al.} \cite{placed2023survey}
        \\
        \hline
    \end{tabular}
    \label{tab:pr_related_review}
\end{table*}
